Can slow pulsars in Milky Way globular clusters form via partial recycling?

Alongside the population of several hundred radio millisecond pulsars currently known in Milky Way globular clusters, a subset of six slowly spinning pulsars (spin periods $0.3-4\,$s) are also observed. With inferred magnetic fields $\gtrsim 10^{11}\,$G and characteristic ages $\lesssim10^8\,$yr, explaining the formation of these apparently young pulsars in old stellar populations poses a major challenge. One popular explanation is that these objects are not actually young but instead have been partially spun up via accretion from a binary companion. In this scenario, accretion in a typical low-mass X-ray binary is interrupted by a dynamical encounter with a neighboring object in the cluster. Instead of complete spin up to millisecond spin periods, the accretion is halted prematurely, leaving behind a ''partially recycled'' neutron star. In this Letter, we use a combination of analytic arguments motivated by low-mass X-ray binary evolution and $N$-body simulations to show that this partial-recycling mechanism is not viable. Realistic globular clusters are not sufficiently dense to interrupt mass transfer on the short timescales required to achieve such slow spin periods. We argue that collapse of massive white dwarfs and/or neutron star collisions are more promising ways to form slow pulsars in old globular clusters.

==> extra_notes.tex <==
People use $\Gamma$ parameter as argument for certain formation scenarios. $\Gamma$ just an $n\sigma v$ estimate so it is a fine proxy for encounter rate (although certainly incomplete relative to real models). However, essentially all proposed formation channels for young pulsars, isolated MSPs, etc scale with $\Gamma$. In this case, $\Gamma$ alone is an incomplete argument. When exploring the detailed physics involved, it appears the partial recycling scenario is not valid. It does indeed scale with $\Gamma$ as Verbunt \& Friere suggest, but the actual encounter timescale required to interrupt spin-up process before millisecond spin periods are reached is far too short ($\lesssim 10^5\,$yr) to be plausible in even in the densest globular clusters. In this case, the WD merger scenario seems more doable. In principle this can be tested in future as our sample of young pulsars in Galactic clusters becomes more complete. In excess of 100 such sources would pose challenge to WD scenario from rates perspective in which case perhaps alternative accretion models are necessary.

Note that https://arxiv.org/pdf/astro-ph/0404136 is a nice review of Galactic GC X-ray sources.

Mass transfer onto a neutron star from a low-mass companion can be driven by nuclear evolution of the companion ($P_{\rm orb} \gtrsim 1\,$d) or by gravitational radiation aided by magnetic braking ($P_{\rm orb} \lesssim 1\,$d) \citep{PhinneyKulkarni1994}. Assuming a $1.2\,M_{\odot}$ neutron star and a $1\,M_{\odot}$ donor, this corresponds to an orbital separation of roughly $5\,R_{\odot}$.

Roughly 13 luminous ($L_x \gtrsim 10^{36}\,$erg/s) low-mass X-ray binaries are observed in Galactic globular clusters \citep{VerbuntLewin2006}. Many low-luminosity ($L_x \lesssim 10^{35}\,$erg/s) X-ray sources are also observed in Galactic clusters \citep{HertzGrindlay1983}, that are generally thought to be accreting white dwarf binaries or potentially neutron star binaries in a quiescent state \citep{Verbunt1984} or even active binaries.

Let's consider the relative ratio of LMXBs to MSPs in globular clusters. 13 bright LXMBs are known. Assuming 

\begin{equation}
    L_{\rm acc} \approx \frac{G M_{\rm ns} \dot{M}}{R_{\rm ns}},
\end{equation}
their luminosities, $L_x \gtrsim 10^{36}\,$erg/s, imply mass accretion rates of roughly $10^{-9}\,M_{\odot}/ \rm{yr}$, or roughly $10\%$ of the Eddington rate for a roughly $1.2\,M_{\odot}$ neutron star.

The mass that must be accreted in order to spin up a neutron star to period $P$ is

\begin{equation}
    \Delta M \approx f 0.08 \Bigg( \frac{P}{2\,\rm{ms}} \Bigg)^{-4/3} M_{\odot}
\end{equation}
\citep{PhinneyKulkarni1994}, where $f \gtrsim 1$ is a factor that depends on the accretion details. In this case, the bright LMXBs observed in globular clusters with inferred accretion rates 
$10^{-9}\,M_{\odot}/ \rm{yr}$ have spin up lifetimes of $\tau_X \approx \Delta M/\dot{M} \approx 10^8(P/2\rm{ms})^{-4/3}\,$yr.  

The ratio of XRB lifetime $\tau_X\approx 10^8\,$yr to MSP lifetime $\tau_{\rm msp} \approx 10^{10}\,$yr implies the Milky Way globular cluster system should contain $100$ times more MSPs than (luminous) low-mass X-ray binaries. The population of $13$ low-mass X-ray binaries observed in Galactic clusters is likely roughly complete, as these sources are bright enough to be observed through the Galaxy. The roughly $300$ known MSPs in Galactic clusters (Freire Pulsar Catalog) is likely incomplete by a factor of a few or more. Thus the expected factor of $100$ overabundance of MSPs relative to XRBs matches observations. Although quiescent X-ray binaries are likely present in globular clusters, this does not affect the discrepancy in birth rates of millisecond pulsars and low-mass X-ray binaries because presumably the neutron stars do not accrete (and get spun up) in their off states.

Adopting a constant $\dot{M} \approx 10^{-9}M_{\odot}/\rm{yr}$, the accretion time to reach spin period of $1\,$s (as observed for the apparently young pulsars of interest) is $\lessim 10^5\,$yr. Thus in order for a partial recycling scenario to provide a viable explanation for these six young pulsars observed, dynamical encounter timescales of order $10^5\,$yr are required in the host cluster in which these objects are found. (Assuming the optimistic case where a dynamical encounter is a sufficient condition to disrupt the the mass transferring binary).

The encounter rate in the center of a cluster like M15 is:

\begin{equation}
         \Gamma_{\rm enc} \approx n \pi a^2 \Bigg(1+\frac{2GM_{\rm tot}}{a \sigma_v^2} \Bigg)\sigma_v  \approx 10^{-10} \Bigg( \frac{n}{10^6\,\rm{pc}^{-3}} \Bigg) \Bigg( \frac{a}{R_{\odot}} \Bigg) \Bigg( \frac{M_{\rm tot}}{3\,M_{\odot}} \Bigg)\Bigg( \frac{\sigma_v}{10\,\rm{km/s}} \Bigg)^{-1} \rm{yr}^{-1}
\end{equation}
(five orders of magnitude too low given LXMB argument above)

%In the classic low-mass X-ray binary scenario for forming millisecond pulsars, a neutron star is spun up as it accretes material from the disk supplied by the donor star. Assuming the material accretes on the neutron star surface ($R_{\rm ns} \approx 10\,$km), the angular momentum of accreted material is roughly $J_{\rm acc}\approx M_{\rm acc} \sqrt{GM_{\rm ns} R_{\rm ns}$. Assuming a neutron star moment of inertia of $I=2M_{\rm ns} R_{\rm ns}^2/5$, the spin angular momentum of a neutron star with spin period $P_{\rm spin}$ is

%\begin{equation}
%    J_{\rm spin} \approx \frac{2}{5} M_{\rm ns} R_{\rm ns}^2 \Big( \frac{2 \pi}{P_{\rm spin}} \Big).
%\end{equation}
%In this case the spin period attained from accretion (adopting the optimistic ``thin disk'' limit where the disk efficiently torques the neutron star) is

%\begin{equation}
%    P_{\rm spin} \approx \frac{4 \pi}{5M_{\rm acc}} \Big( \frac{M_{\rm ns} R_{\rm ns}^3}{G} \Big)^{1/2} \approx 10 \Big( \frac{M_{\rm acc}}{0.02\,M_{\odot}} \Big)^{-1} \rm{ms},
%\end{equation}
%found by equating $J_{\rm spin}$ and $J_{\rm acc}$. In order to achieve $1\,$s spin periods comparable to those observed for the apparently young pulsars, only $\sim10^{-4}M_{\odot}$ can be accreted. Assuming an accretion rate of roughly $10^{-9}M_{\odot}\,\rm{yr}^{-1}$ onto the neutron star, this would require a spin-up time scale of only $10^5\,$yr, orders of magnitude less than the typical time scale. In this case, even if a dynamical encounters does occur which may interupt mass transfer in a LMXB, such an encounter will likely occur only after the neutron star has already been spun up to millisecond spin periods. In this case, a single MSP would be formed Indeed many such objects are observed in Galactic globular clusters, notably core-collapsed globular clusters.

Also... can we argue that if partial recycling is valid, there should be 10x as many 100ms and 100x as many 10ms pulsars relative to the 1s young pulsars? This is clearly not the case. I think we still need to be able to explain the intermediate spin period pulsars with periods of 50 ms etc. Could these be partial spin up? Certainly more plausible since these require spin up times factor of 50-100x longer which gives you much longer time to have encounter.

Verbunt and Friere say, ``The distribution of intermediate pulse periods forms a bridge between the shortest pulse periods and the longest pulse periods, which suggests that the latter are the tail of a continuous distribution rather than a separate group.'' It is a good point which we need to discuss.

\textbf{Also look at Eq 5 of their paper which also raises interesting challenge to partial recycling model that they kind of brush under the rug. I think there is also discussion in Tauris 2012 you should read...}

``Assuming that the pulsars in GCs are young, Boyles et al. (2011) estimate that a birth rate of 1 every $10^4$ yr is required to explain the observed number of young pulsars in the GC system.'' Note sure I understand that rate... is this accounting for detection biases? 

I think the most obvious way to make partial recycling viable is if in fact XRBs spend most of their time accreting at some very low rate (that could presumably spin up to 1 s spin periods over 1 Gyr or more) and then only shine very brightly for very small fraction of their lifetime. In that case, the ratio of MSPs to bright XRBs would have to be MUCH larger. If in the future a much larger number of MSPs and also young pulsars in clusters are observed this may favor the partial recycling scenario. I think we can make nice schematic figure showing the spin up time, the encounter time, and the fraction of MSPs, young pulsars, and XRBs to show regime where partial recycling is viable...

\citet{Heinke2003} points out that globular cluster qLMXBs range in luminosity from $10^{32}\,$erg/s up to a few $\times 10^{33}\,$erg/s, corresponding to accretion rates of roughly at least a few$\times 10^{-12}M_{\odot}/\rm{yr}^{-1}$ (I think accounting for some efficiency factor in Eq 1). qLMXBs can be separated out from the other low-luminosity X-ray sources (e.g., CVs) because they have softer spectra \citep[e.g.,][]{Pooley2003}. Critically, quiescent LMXBs below $10^{32}\,$erg/s \textit{would have been identifiable in most clusters}, so the luminosity cutoff implies a lower limit to the time-averaged mass accretion rate. You should confirm this with Craig and/or Jay. Note that this range of qLMXB luminosities is consistent with the \citet{Brown1998} model for qLMXB emission, because higher mass-transfer rates would lead to persistent systems and significantly lower rates would probably require systems older than a Hubble time.

I think this accretion limit for qLMXBs alone may kill this story because $\dot{M} > 10^{-12}M_{\odot}/\rm{yr}^{-1}$ would require encounter timescale of $<10^8\,$yr which is not achieved even in the absolute densest globular clusters. 


\textit{Other argument: Encounter time is longer than total mass transfer time:} 

Perhaps the above point can be avoided if the mass accretion rate is significantly lower than Eddington rate or if the spin-up of the neutron star is highly inefficient. In either of these cases, it may take the neutron star much longer to spin up, perhaps allowing for sufficient time for a dynamical encounter to occur after the neutron star has been only partially recycled. In this slow accretion rate limit, a separate limit becomes relevant based on the mass transfer lifetime of the donor star.

For a main sequence star, $\dot{M}\approx10^{-9}\,M_{\odot}\rm{yr}^{-1}$ and the mass transfer time $t_{\rm MT}$ is set by the time to deplete the mass of the star completely $t_{\rm MT} \approx M/\dot{M} \approx 10^9\,$yr. This timescale is shorter than the typical encounter timescale (roughly $10^{10}\,$yr), thus encounters rarely can interrupt mass transfer for main sequence stars.

For giant branch stars, the encounter timescale is shorter because the stellar radius is larger (binary fills Roche lobe at larger orbital separation). However, the mass transfer timescale here is set by the evolutionary time of the giant, $\lesssim 10^7\,$yr. Assuming $a\approx10^2\,R_{\odot}$ for a solar mass AGB star, the encounter timescale is roughly $10^8\,$yr. Again, the encounter timescale is much longer than the typical mass transfer time, indicating interruption of mass transfer by dynamical encounters is rare.

Also note that if we invoke highly inefficient accretion onto the neutron star, then we run into a separate problem: we never produce MSPs. For example, in order for a main-sequence star to spin up a neutron star to millisecond spin period in $10^9\,$yr, a minimum accretion rate of roughly $10^{-11}M_{\odot}\rm{yr}^{-1}$ is required. 


\textit{Alternative: Formation via massive white dwarf mergers -- } 


\textit{Observational tests --}
Using FAST Observations, \citet{Yin+2024} suggested that the escaped velocities of the clusters work better (which is just another parameter, but it shows that even observational the encounter rates don't really work). And 47 Tuc has more pulsars observed than predicted by the encounter rate in \citet{Turk_Lorimer_2013} (although this paper does not give uncertainties.)
